High Fidelity Video Prediction with Large Stochastic Recurrent Neural Networks

Predicting future video frames is extremely challenging, as there are many factors of variation that make up the dynamics of how frames change through time. Previously proposed solutions require complex inductive biases inside network architectures with highly specialized computation, including segmentation masks, optical flow, and foreground and background separation. In this work, we question if such handcrafted architectures are necessary and instead propose a different approach: finding minimal inductive bias for video prediction while maximizing network capacity. We investigate this question by performing the first large-scale empirical study and demonstrate state-of-the-art performance by learning large models on three different datasets: one for modeling object interactions, one for modeling human motion, and one for modeling car driving.

==> figures/combined_dynamic_eval.tex <==
\begin{figure}[htp!]
    \centering
    \hspace{-8pt}
	\includegraphics[width=.35\linewidth]{figures/plots/towel/fvd.jpg} \hspace{-15pt}
	\includegraphics[width=.35\linewidth]{figures/plots/humans/fvd.jpg} \hspace{-15pt}
	\includegraphics[width=.35\linewidth]{figures/plots/driving/fvd.jpg}
	\caption{Video dynamics evaluation. The figure on the left illustrates how Frechet Video Distance decreases as model capacity is increased (lower means better).}
    \label{fig:combined_dyn}
\end{figure}


==> figures/combined_dynamic_eval_all.tex <==
\begin{figure}[htp!]
    \centering
    \hspace{-8pt}
	\includegraphics[width=.35\linewidth]{figures/plots/towel/fvd_all.pdf} \hspace{-15pt}
	\includegraphics[width=.35\linewidth]{figures/plots/humans/fvd_all.pdf} \hspace{-15pt}
	\includegraphics[width=.35\linewidth]{figures/plots/driving/fvd_all.pdf}
	\caption{Video dynamics evaluation (lower is better). The figures illustrate how Frechet Video Distance decreases as model capacity is increased. Note that all models (SVG', CNN, and LSTM) are generated using the same $M$ and $K$ combination as described in Section~\ref{sec:method}, which is why the smaller architectures (CNN and LSTM) naturally have fewer parameters.}
    \label{fig:combined_dyn_all}
    \vspace{-0.1in}
\end{figure}

==> figures/driving128_figure.tex <==
\begin{figure}[thbp!]%[!t]
    % \vspace{-8pt}
    \hspace*{-.5cm}
    \centering
	\begin{subfigure}{0.1\linewidth}
        \raggedleft
        \rotatebox{90}{
        \hspace{-.5cm}
        \parbox{1.6cm}{\centering Smallest model \\ (Baseline)}
        \parbox{1.6cm}{\centering Biggest model \\ (Ours)}
        \parbox{1.6cm}{\centering Groundtruth}
        }
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \caption*{t=8}
        \vspace{-7pt}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0007_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0049/0007.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0007.jpg}
	\end{subfigure} 
    \begin{subfigure}{0.12\linewidth}
        \caption*{t=11}
        \vspace{-7pt}  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0010_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0049/0010.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0010.jpg}
	\end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \caption*{t=14}
        \vspace{-7pt}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0013_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0049/0013.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0013.jpg}
	\end{subfigure} 
    \begin{subfigure}{0.12\linewidth}
        \caption*{t=17}
        \vspace{-7pt}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0016_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0049/0016.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0016.jpg}
	\end{subfigure}
	\begin{subfigure}{0.12\linewidth}
        \caption*{t=20}
        \vspace{-7pt}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0019_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0049/0019.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0019.jpg}
	\end{subfigure}
	\begin{subfigure}{0.12\linewidth}
        \caption*{t=23}
        \vspace{-7pt}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0022_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0049/0022.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0022.jpg}
	\end{subfigure}
	\begin{subfigure}{0.12\linewidth}
        \caption*{t=26}
        \vspace{-7pt}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0025_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0049/0025.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0049/0025.jpg}
	\end{subfigure}

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \hspace{-14pt}
%     \centering
% 	\begin{subfigure}{0.1\linewidth}
%         \raggedleft
%         \rotatebox{90}{
%         \hspace{-.3cm}
%         \parbox{1.6cm}{\centering Smallest model \\ (Baseline)}
%         \parbox{1.6cm}{\centering Biggest model \\ (Ours)}
%         \parbox{1.6cm}{\centering Groundtruth}
%         }
%     \end{subfigure}
%     \begin{subfigure}{0.12\linewidth}
%         \vspace{5pt}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0007_gt.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0140/0007.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0007.jpg}
% 	\end{subfigure} 
%     \begin{subfigure}{0.12\linewidth}
%         \vspace{5pt}  		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0010_gt.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0140/0010.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0010.jpg}
% 	\end{subfigure}
%     \begin{subfigure}{0.12\linewidth}
%         \vspace{5pt}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0013_gt.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0140/0013.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0013.jpg}
% 	\end{subfigure} 
%     \begin{subfigure}{0.12\linewidth}
%         \vspace{5pt}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0016_gt.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0140/0016.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0016.jpg}
% 	\end{subfigure}
% 	\begin{subfigure}{0.12\linewidth}
%         \vspace{5pt}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0019_gt.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0140/0019.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0019.jpg}
% 	\end{subfigure}
% 	\begin{subfigure}{0.12\linewidth}
%         \vspace{5pt}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0022_gt.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0140/0022.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0022.jpg}
% 	\end{subfigure}
% 	\begin{subfigure}{0.12\linewidth}
%         \vspace{5pt}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0025_gt.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_big/0140/0025.jpg}
%   		\includegraphics[width=1\linewidth]{figures/images/driving128_small/0140/0025.jpg}
% 	\end{subfigure}

    \caption{KITTI driving qualitative evaluation. High resolution video (frame size of 128x128) comparison between smallest model and largest model we were able to train (M=3, K=3). For best viewing and more results, please visit our website \url{https://cutt.ly/QGuCex}.}
\label{fig:qualitative_driving128}
\end{figure}



==> figures/driving128_plots.tex <==
\begin{figure}[htp!]
    \centering
	\includegraphics[width=.4\linewidth]{figures/plots/driving128/cosine_sim.jpg} \hspace{.8cm}
	\includegraphics[width=.4\linewidth]{figures/plots/driving128/fvd.jpg}
	\caption{KITTI Driving quantitative evaluation.}
\label{fig:quant_kitti}
\end{figure}


==> figures/driving_dynamic_eval.tex <==
\begin{figure}[htp!]
    \centering
    \hspace{-8pt}
	\includegraphics[width=.5\linewidth]{figures/plots/driving/fvd.jpg}
	\includegraphics[width=.5\linewidth]{figures/driving_chart.pdf}
	\caption{KITTI driving video dynamics evaluation. The figure on the left illustrates how Frechet Video Distance decreases as model capacity is increased (lower means better). The pie chart on the right indicates the percentage of AMT workers that prefer our model over the baseline, prefer the baseline over our model, and cannot tell the difference between the two.}
    \label{fig:dyn_kitti}
\end{figure}



==> figures/humans128_figure.tex <==
\begin{figure}[thbp!]%[!t]
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \hspace{-14pt}
    \centering
	\begin{subfigure}{0.1\linewidth}
        \raggedleft
        \rotatebox{90}{
        \hspace{-.3cm}
        \parbox{1.6cm}{\centering Smallest model \\ (Baseline)}
        \parbox{1.6cm}{\centering Biggest model \\ (Ours)}
        \parbox{1.6cm}{\centering Groundtruth}
        }
    \end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \vspace{5pt}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0007_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_big/0229/0007.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0007.jpg}
	\end{subfigure} 
    \begin{subfigure}{0.12\linewidth}
        \vspace{5pt}  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0010_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_big/0229/0010.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0010.jpg}
	\end{subfigure}
    \begin{subfigure}{0.12\linewidth}
        \vspace{5pt}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0013_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_big/0229/0013.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0013.jpg}
	\end{subfigure} 
    \begin{subfigure}{0.12\linewidth}
        \vspace{5pt}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0016_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_big/0229/0016.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0016.jpg}
	\end{subfigure}
	\begin{subfigure}{0.12\linewidth}
        \vspace{5pt}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0019_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_big/0229/0019.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0019.jpg}
	\end{subfigure}
	\begin{subfigure}{0.12\linewidth}
        \vspace{5pt}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0022_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_big/0229/0022.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0022.jpg}
	\end{subfigure}
	\begin{subfigure}{0.12\linewidth}
        \vspace{5pt}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0025_gt.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_big/0229/0025.jpg}
  		\includegraphics[width=1\linewidth]{figures/images/humans128_small/0229/0025.jpg}
	\end{subfigure}

    \caption{Human 3.6M qualitative evaluation. High resolution video (frame size of 128x128) comparison between smallest model and largest model we were able to train (M=3, K=3). For best viewing and more results, please visit our website \url{https://cutt.ly/QGuCex}.}
\label{fig:qualitative_humans128}
\end{figure}


==> figures/humans128_plots.tex <==
\begin{figure}[htp!]
    \centering
	\includegraphics[width=.4\linewidth]{figures/plots/humans128/cosine_sim.jpg} \hspace{.8cm}
	\includegraphics[width=.4\linewidth]{figures/plots/humans128/fvd_all.jpg}
	\caption{Human 3.6M quantitative evaluation.}
\label{fig:quant_h36m}
\end{figure}


==> figures/humans_dynamic_eval.tex <==
\begin{figure}[htp!]
    \centering
    \hspace{-8pt}
    \mbox{
        \centering
     	\includegraphics[width=.5\linewidth]{figures/plots/humans/fvd.jpg}
        \includegraphics[width=.5\linewidth]{figures/humans_chart.pdf}
    }

	\caption{Human 3.6M video dynamics evaluation. The figure on the left illustrates how Frechet Video Distance decreases as model capacity is increased (lower means better). The pie chart on the right indicates the percentage of AMT workers that prefer our model over the baseline, prefer the baseline over our model, and cannot tell the difference between the two.}
    \label{fig:dyn_humans}
\end{figure}



==> figures/towel_dynamic_eval.tex <==
\begin{figure}[htp!]
    \centering
    \hspace{-8pt}
	\includegraphics[width=.5\linewidth]{figures/plots/towel/fvd.jpg}
	\includegraphics[width=.5\linewidth]{figures/towel_chart.pdf}
	\caption{Towel pick video dynamics evaluation. The figure on the left illustrates how Frechet Video Distance decreases as model capacity is increased (lower means better). The pie chart on the right indicates the percentage of AMT workers that prefer our model over the baseline, prefer the baseline over our model, and cannot tell the difference between the two.}
    \label{fig:dyn_towel}
\end{figure}



==> sections/5_experiments_old.tex <==
\cutsectionup
\section{Experiments}
\cutsectiondown

% Dataset description, challenges, why we use them, preprocessing, train/test splits
In this section, we evaluate our method on three different datasets, each with different challenges. 

\textbf{Object interactions.}
% We use the action-conditioned robot push dataset from~\citet{softmotion} and towel pick dataset from ~\citet{frederik}. These datasets contain a robot arm that is interacting with object.
We use the action-conditioned towel pick dataset from~\citet{frederik} to evaluate how our models perform with standard object interactions. This dataset contains a robot arm that is interacting with towel objects. Even though this dataset uses action-conditioning, stochastic video prediction is still required for this task. This is because the motion of the objects is not fully determined by the actions (the movements of the robot arm), but also includes factors such as friction and the objects' current state. For this dataset, we resize the original resolution of 48x64 to 64x64. For evaluation, we use the first 256 videos in the test set as defined by~\citet{frederik}.

\textbf{Structured motion.} We use the Human 3.6M dataset~\citep{human36m} to measure the ability of our models to predict structured motion. This dataset is comprised of humans performing actions inside a room (walking around, sitting on a chair, etc.). Human motion is highly structured (i.e., many degrees of freedom), and so, it is difficult to model. We use the train/test split from~\citet{villegas17hierchvid}. For this dataset, we resize the original resolution of 1000x1000 to 64x64.

\textbf{Partial observability.} We use the KITTI driving dataset~\citep{kitti} to measure how our models perform in conditions of partial observability. This dataset contains driving scenes taken from a front camera view of a car driving in the city, residential neighborhoods, and on the road. The front view camera of the vehicle causes partial observability of the vehicle environment, which requires a model to generate seen and unseen areas when predicting future frames. We use the train/test split from~\citet{prednet} in our experiments. We extract 30 frame clips and skip every 5 frames from the test set so that the test videos do not significantly overlap, which gives us 148 test clips in the end. For this dataset, we resize the original resolution of 128x160 to 64x64.

% Evaluation metrics description and why we use them (don't forget to include copy last frame evaluation?)
\cutsubsectionup
\subsection{Evaluation Metrics}
\cutsubsectiondown
We perform a rigorous evaluation using five different metrics: 
Peak Signal-to-Noise Ratio (PSNR), Structural Similarity (SSIM), VGG Cosine Similarity, Fr\'echet Video Distance (FVD)~\citep{fvd}, and human evaluation from Amazon Mechanical Turk (AMT) workers.
We perform these evaluations on all models described in Section~\ref{sec:method}: our baseline (denoted as SVG'), the recurrent deterministic model (denoted as LSTM), and the encoder-decoder CNN model (denoted as CNN).
\cutsubsectionup
\subsubsection{Frame-wise evaluation}
\cutsubsectiondown
We use three different metrics to perform frame-wise evaluation: PSNR, SSIM, and VGG cosine similarity. 
PSNR and SSIM perform a pixel-wise comparison between the predicted frames and generated frames, effectively measuring if the exact pixels have been generated.
VGG Cosine Similarity has been used in prior work~\citep{alexlee} to compare frames in a perceptual level. VGGnet~\citep{vggnet} is used to extract features from the predicted and ground-truth frames, and cosine similarity is performed at feature-level. Similar to~\citet{Kumar19,mohammad,alexlee}, we sample 100 future trajectories per video and pick the highest scoring trajectory as the main score. 
\cutsubsectionup
\subsubsection{Dynamics-based evaluation}
\cutsubsectiondown
We use two different metrics to measure the overall realism of the generated videos: FVD and human evaluations. FVD, a recently proposed metric for video dynamics accuracy, uses a 3D CNN trained for video classification to extract a single feature vector from a video. Analogous to the well-known FID~\citep{fid}, it compares the distribution of features extracted from ground-truth videos and generated videos. Intuitively, this metric compares the quality of the overall predicted video dynamics with that of the ground-truth videos rather than a per-frame comparison. For FVD, we also sample 100 future trajectories per video, but in contrast, all 100 trajectories are used in this evaluation metric (i.e., not just the max, as we did for VGG cosine similarity).

We also use Amazon Mechanical Turk (AMT) workers to perform human evaluations. The workers are presented with two videos (baseline and largest models) and asked to either select the more realistic video or mark that they look about the same. We choose the videos for both models by selecting the highest scoring videos in terms of the VGG cosine similarity with respect to the ground truth. 
%  We ask the workers data-specific realism questions. %TODO(HK): what are these questions? shoud we put this in the supplementary material?
We use 10 unique workers per video and choose the selection with the most votes as the final answer.
Finally, we also show qualitative evaluations on pairs of videos, also selected by using the highest VGG cosine similarity scores for both the baseline and the largest model. % TODO(HK): clarify if the qualitative evals shown below are selected randomly? or cherry picked
We run the human perception based evaluation on the best two architectures we scale up.

% Network architecture description maybe in supplementary material? (mention fully-convolutional architecture being used number of convolutional layers in encoder/decoder, etc)
% Describe the K/M for increasing the number of parameters

\input{figures/combined_dynamic_eval_all.tex}
\input{tables/mturk_together.tex}

% Robot experiments (mention that the examples visualized are the top based on cosine sim) and that modified svg to take in actions
\cutsubsectionup
\subsection{Robot Arm}
\cutsubsectiondown
For this dataset, we perform action-conditioned video prediction. We modify the baseline and large models to take in actions as additional input to the video prediction model. Action conditioning does not take away the inherent stochastic nature of video prediction due to the dynamics of the environment. During training time, the models are conditioned on 2 input frames and predict 10 frames into the future. During test time, the models predict 18 frames into the future.

\cutparagraphup
\paragraph{Dynamics-based evaluation.}
% We first evaluate the action conditioned video prediction models using FVD to measure the realism in the dynamics. In Figure~\ref{fig:combined_dyn}, we can see that the FVD scores continuously drop as the model capacity is increased. This is a signal that the robotic arm dynamics gets closer to the true dynamics as seen in the ground-truth data, and also, the interactions with the environment become more accurate.
We first evaluate the action-conditioned video prediction models using FVD to measure the realism in the dynamics. In Figure~\ref{fig:combined_dyn_all} (left), we present the results of scaling up the three models described in Section~\ref{sec:method}. Firstly, we see that our baseline architecture does indeed improve dramatically as capacity is increased. Secondly, for our ablative experiments, we notice that capacity does seem to improve the performance of the vanilla CNN architecture. Interestingly, by increasing the capacity of the CNN architecture to approximately 100M parameters, it approaches the performance of the original SVG' architecture at around 30M parameters. However, as capacity increases, the lack of recurrence heavily affects the performance of the vanilla CNN architecture in comparison with the models that do have an LSTM.
Both the LSTM model and SVG' perform similarly well, with LSTM model performing slightly better. This makes sense as the deterministic LSTM model is more likely to produce videos closer to the ground truth; however, the stochastic component is still quite important as a good video prediction model must be both realistic and capable of handling multiple possible futures. 
Finally, we use human evaluations through Amazon Mechanical Turk to compare our biggest models with the corresponding baselines. We ask workers to focus on how realistic the interaction between the robot arm and objects looks. As shown in Table~\ref{table:mturk_together}, the largest SVG' is preferred 68.8\% of the time vs 25.8\% of the time for the baseline (right), and the largest LSTM model is preferred 90.2\% of the time vs 9.0\% of the time for the baseline (left). 

%We hypothesize that the baseline is preferred 25.8\% of the time because, as it can be seen in the supplementary videos, sometimes the largest capacity model sometimes drops objects when it should not. This may be due to internal miscalculations of the objects' physics by the model.
% \input{figures/towel_dynamic_eval.tex}

\cutparagraphup
\paragraph{Frame-wise evaluation.}
% Next, we perform per-frame evaluation using PSNR, SSIM and VGG Cosine Similarity. These metrics measure how accurately the robot arm moves and interacts with its surroundings. As shown in Figure~\ref{fig:frame_towel}, frame wise performance improves as the capacity of the model increases. This means that the predicted pixels are more accurate for the model with the most capacity compared to the smallest (baseline) model. However, frame wise accuracy does not necessarily imply that the overall dynamics of the generated videos are accurate.
Next, we use FVD to select the best models from CNN, LSTM, and SVG', and perform frame-wise evaluation on each of these three models. 
%Since models that copy background pixels perfectly can perform well on these frame-wise evaluation metrics, we also include a simple baseline where the last observed frame is copied through time. 
Since models that copy background pixels perfectly can perform well on these frame-wise evaluation metrics, in the supplementary material we also discuss a comparison against a simple baseline where the last observed frame is copied through time. 
%
From Figure~\ref{fig:frame_towel}, we can see that the CNN model performs much worse than the models that have recurrent connections. This is a clear indication that recurrence is necessary to predict future frames, and capacity cannot make up for it. Both LSTM and SVG perform similarly well, however, towards the end, SVG slightly outperforms LSTM. The full evaluation on all capacities for SVG', LSTM, and CNN is presented in the supplementary material.

\input{figures/towel_frame_eval_all.tex}

\cutparagraphup
\paragraph{Qualitative evaluation.} In Figure~\ref{fig:qualitative_towel}, we show example videos from the smallest SVG' model, the largest SVG' model, and the ground truth. The predictions from the small baseline model are blurrier compared to the largest model, while the edges of objects from the larger model's predictions stay continuously sharp throughout the entire video. This is clear evidence that increasing the model capacity enables more accurate modeling of the pick up dynamics. For more videos, please visit our anonymous website \url{https://bit.ly/2LWepP2}.
\input{figures/towel_figure.tex}

% Our results confirm that model capacity is an important factor to making better video prediction models, even on a dataset that is relatively easy to model. 

% \newpage
% Humans experiments (mention that the examples visualized are the top based on cosine sim). Also include the long-term prediction experiments?
\cutsubsectionup
\subsection{Human Activities} \label{sec:humans}
\cutsubsectiondown
For this dataset, we perform action-free video prediction. We use a single model to predict all action sequences in the Human 3.6M dataset. During training time, the models are conditioned on 5 input frames and predict 10 frames into the future. At test time, the models predict 25 frames.

% \cutparagraphup \paragraph{Dynamics-based evaluation.} First, we evaluate the predicted human structured dynamics in terms of dynamic realism. Like the results from the robotics dataset, Figure~\ref{fig:combined_dyn_all} (middle) shows FVD decreasing as capacity increases, indicating that the predicted frames reflect more accurate human dynamics. Secondly, in our human evaluations for SVG, 95.8\% of the AMT workers agree that the bigger model has more realistic videos in comparison to the smaller model. Our results, especially the strong agreement from our human evaluations, show that high capacity models are better equipped to handle the complex structured dynamics in human videos. \todo{add deterministic model results}

\cutparagraphup \paragraph{Dynamics-based evaluation.}
We evaluate the predicted human motion with FVD (Figure~\ref{fig:combined_dyn_all}, left). The performance of the CNN model is poor in this dataset, and increasing the capacity of the CNN does not lead to any increase in performance. We hypothesize that this is because the lack of action conditioning and the many degrees of freedom in human motion makes it very difficult to model with a simple encoder-decoder CNN. However, after adding recurrence, both LSTM and SVG' perform significantly better, and both models' performance become better as their capacity is increased. Secondly, in our human evaluations for SVG', 95.8\% of the AMT workers agree that the bigger model has more realistic videos in comparison to the smaller model, and for LSTM, 98.7\% of the workers agree that the LSTM largest model is more realistic. Our results, especially the strong agreement from our human evaluations, show that high capacity models are better equipped to handle the complex structured dynamics in human videos. 

% \input{figures/humans_dynamic_eval.tex}

% \cutparagraphup \paragraph{Frame-wise evaluation.} Next, we evaluate each of the predicted frames against the ground-truth video. In contrast to the dynamics-based evaluations, we see that these results do not reflect the same findings. This happens because the background not being perfectly predicted and it takes up a large portion of the frame. We include a baseline based on simply copying the last observed frame which translates into perfect background prediction. Since the background in this dataset is This claim can also be verified in the videos provided in the supplementary material, as well as, the AMT and FVD evaluation above.

\cutparagraphup 
\paragraph{Frame-wise evaluation.} Similar to the previous per-frame evaluation, we select the best performing models in terms of FVD and perform a frame-wise evaluation. In Figure~\ref{fig:frame_humans}, we see an interesting behavior. This dataset is mostly made of static background and the human takes a very small area of it. Therefore, the per-frame evaluation favors perfect reconstruction of the background, and thus, the "copy last frame" baseline outperforms all the methods (see the supplementary material), but it obviously performed poorly with the dynamics-based evaluation. Finally, similar to the previous results, we see the recurrent models outperform the CNN model.
We present the full evaluation on all capacities for SVG’, LSTM, and CNN in the supplementary material.
\input{figures/humans_frame_eval_all.tex}

\cutparagraphup
\paragraph{Qualitative evaluation.} Figure~\ref{fig:qualitative_humans} shows a comparison between the smallest and largest stochastic models. In the video generated by the smallest model, the shape of the human is not well-defined at all, while the largest model is able to clearly depict the arms and the legs of the human. Moreover, our large model is able to successfully predict the human's movement throughout all of the frames into the future. The predicted motion is close to the ground-truth motion providing evidence that being able to model more factors of variation with larger capacity models can enable accurate motion identification and prediction. For more videos, please visit our anonymous website \url{https://bit.ly/2LWepP2}.
\input{figures/humans_figure.tex}

% Driving experiments (mention that the examples visualized are the top based on cosine sim)
\cutsubsectionup
\subsection{Car Driving}
\cutsubsectiondown
For this dataset, we also perform action-free video prediction. During training time, the models are conditioned on 5 input frames and predict 10 frames into the future. At test time, the models predict 25 frames into the future. This video type is the most difficult to predict. It requires the model to be able to hallucinate unseen parts in the video given the observed parts.

% \cutparagraphup 
% \paragraph{Dynamics-based evaluation.} As in previous experiments, we first evaluate videos in terms of dynamics. From Figure~\ref{fig:combined_dyn_all} (right), we can see an extreme gain as the capacity of the model increases in terms of FVD. In addition, 99.3\% of the AMT workers agree that our largest capacity model generates more realistic videos in comparison to the baseline model. Finally, 0\% of the workers think that any of the comparisons look about the same. 
% \input{figures/driving_dynamic_eval.tex}

\cutparagraphup
\paragraph{Dynamics-based evaluation.} We see very similar results to the previous dataset when measuring the realism of the videos. From Figure~\ref{fig:combined_dyn_all} (right), we see a large improvement in FVD as the capacity of the model increases for both LSTM and SVG'. However, we see a similarly poor performance for the CNN architecture as in Section~\ref{sec:humans}, where capacity does not really help at all. One interesting thing to note is that the LSTM model starts to decrease in FVD score rapidly, which is likely related to the differences in a deterministic vs. stochastic architecture discussed in the previous sections, where the scores for a deterministic model can improve rapidly by simply fitting the ground truth in a deterministic way. Finally, for human evaluations, we see in Table~\ref{table:mturk_together} that the largest capacity SVG' model is preferred by human raters 99.3\% of the time (right), and the largest capacity LSTM model (left) is also preferred by human raters 99.3\% time (left).

% \cutparagraphup\paragraph{Frame-wise evaluation} Now, when we evaluate based on frame-wise accuracy, we see a similar but not exactly the same behavior to the Human 3.6M experiments. In this dataset, the models are often required to predict frames on the right side of frame view. This requires the model to guess what is in the completely unseen area. This can result in large errors when the model guesses correctly regardless of the realism in the overall video dynamics. Again, this can be verified by the FVD and AMT evaluation results. We provide all video comparisons in the supplementary material.

\cutparagraphup
\paragraph{Frame-wise evaluation} Now, when we evaluate based on frame-wise accuracy, we see similar but not exactly the same behavior as the experiments in Section~\ref{sec:humans}. The CNN architecture performs poorly as expected, however, LSTM and SVG' perform similarly well.
% For this dataset, we do not present a copy last frame baseline because most pixels move in contrast to the robot arm and Human 3.6M dataset.
% Surprisingly, we see that the copy last frame baseline does fairly well, especially on VGG cosine similarity. This may happen because the background pixels (the sky and street) take up more space than the vehicles. 

%Additionally, in this dataset the models are often required to predict out-of-view frames. This requires the model to guess what is in the completely unseen area. This can result in large errors when the model guesses correctly regardless of the realism in the overall video dynamics. All of this put together results in the illusion of good performance by the copy last frame baseline.

\input{figures/driving_frame_eval_all.tex}

% \cutparagraphup\paragraph{Qualitative evaluation.} In Figure~\ref{fig:qualitative_driving}, we can clearly see the difference in prediction quality. The baseline model starts becoming blurry as the predictions move forward in the future, and important features like the lane markings disappear. However, our biggest capacity model makes very sharp predictions that look realistic in comparison to the ground-truth. This result provides evidence that the largest capacity model can hallucinate sharp unseen frame dynamics multiple frames into the future without the need to use any adversarial training as in other methods. For more videos, please visit our anonymous website \url{https://bit.ly/2LWepP2}.
% \input{figures/driving_figure.tex}

\input{figures/driving_figure.tex}

\cutparagraphup
\paragraph{Qualitative evaluation.} 
In Figure~\ref{fig:qualitative_driving}, we show a comparison between the largest stochastic model and its baseline. The baseline model starts becoming blurry as the predictions move forward in the future, and important features like the lane markings disappear. However, our biggest capacity model makes very sharp predictions that look realistic in comparison to the ground-truth. 



==> tables/baselines.tex <==

\begin{table}[h!] 
\centering
% \small
\setlength{\tabcolsep}{3pt}
\vspace{10pt}
\begin{tabular}{l||c||c||c || c || c}
\Xhline{4\arrayrulewidth}
\Xhline{4\arrayrulewidth}
Dataset & \makecell{SVG' (largest)} & \makecell{LSTM' (largest)} & \makecell{SVG' (baseline)} & \makecell{SV2P} & \makecell{SAVP} \\
\Xhline{4\arrayrulewidth}

\Xhline{4\arrayrulewidth}
Human 3.6M 
& \makecell{429.88} 
& \makecell{458.77} 
& \makecell{682.08} 
& \makecell{todo} 
& \makecell{todo} \\

\Xhline{4\arrayrulewidth}
KITTI 
& \makecell{1217.25} 
& \makecell{1159.25} 
& \makecell{2264.91} 
& \makecell{todo} 
& \makecell{todo} \\

\Xhline{4\arrayrulewidth}
BAIR 
& \makecell{93.71} 
& \makecell{100.04} 
& \makecell{189.91}
& \makecell{todo} 
& \makecell{todo} \\

\Xhline{4\arrayrulewidth}
\Xhline{4\arrayrulewidth}
\end{tabular}
\vspace{12pt}
\caption{Fr\'echet Video Distance (FVD) evaluation of the effects of the number of context frames in the action-free datasets (Human 3.6M and KITTI). We compare models with different number of context frames and prediction of 20 frames.}
\vspace{-.1in}
\label{table:context_actionfree_fvd}
\end{table}

==> tables/mturk_deterministic.tex <==
\begin{table}[t] 
\centering
% \small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\Xhline{4\arrayrulewidth}
Dataset & Biggest model & Baseline & About the same  \\
\Xhline{4\arrayrulewidth}
Towel Pick & \textbf{90.2}\% & 9.0\% & 0.8\% \\
Human 3.6M & \textbf{98.7}\% & 1.3\% & 0.0\% \\
KITTI Driving & \textbf{99.3}\% & 0.7\% & 0.0\% \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\caption{Deterministic models comparison. }
\vspace{-12pt}
\label{table:mturk_det}
\end{table}



==> tables/mturk_stoch_vs_det.tex <==
\begin{table}[t] 
\centering
% \small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\Xhline{4\arrayrulewidth}
Dataset & Biggest stochastic & Biggest deterministic & About the same  \\
\Xhline{4\arrayrulewidth}
Towel Pick & - & - & - \\
Human 3.6M & - & - & - \\
KITTI Driving & - & - & - \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\caption{Stochastic vs deterministic models. }
\vspace{-12pt}
\label{table:m_turk}
\end{table}



==> tables/mturk_stochastic.tex <==
\begin{table}[t] 
\centering
% \small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\Xhline{4\arrayrulewidth}
Dataset & Biggest model & Baseline & About the same  \\
\Xhline{4\arrayrulewidth}
Towel Pick & \textbf{68.8}\% & 25.8\% & 5.5\% \\
Human 3.6M & \textbf{95.8}\% & 3.4\% & 0.8\% \\
KITTI Driving & \textbf{99.3}\% & 0.7\% & 0.0\% \\
\Xhline{4\arrayrulewidth}
\end{tabular}
\caption{Stochastic models comparison. }
\vspace{-12pt}
\label{table:mturk_stoch}
\end{table}

